UNDIAL: Self-Distillation with Adjusted Logits for Robust Unlearning in Large Language Models

Mitigating the retention of sensitive or private information in large language models is essential for enhancing privacy and safety. Existing unlearning methods, like Gradient Ascent and Negative Preference Optimization, directly tune models to remove unwanted information. However, these methods often become unstable because they fine-tune by maximizing cross-entropy loss, which is the opposite of traditional loss minimization in learning. This reversal creates instability, especially on larger datasets, as the model struggles to balance unlearning with maintaining language capacity, leading to over-unlearning. In this paper, we introduce UnDIAL (Unlearning via Self-Distillation on Adjusted Logits), a novel and robust unlearning method. Our approach leverages self-distillation to adjust logits and selectively reduce the influence of targeted tokens. This technique ensures smooth convergence and avoids catastrophic forgetting, even in challenging unlearning tasks with large datasets and sequential unlearning requests. Extensive experiments show that UnDIAL can achieve both robustness in unlearning and scalability while maintaining stable training dynamics and resilience to hyperparameter tuning.

==> table/NLU_benchmark.tex <==
\begin{table*}[t]
\centering


\begin{tabular}{|l|r|r|r r r|r r r r r r|}
\hline
Method & Coeff & EL\_3($\downarrow$) & MAUVE & PPL($\downarrow$) & Rep\_3($\downarrow$) & Piqa & ARC & Copa & Wino. & Pubmed & Hella. \\
\hline

GPT-Neo & - & 0.202 & 0.718 & 17.192 & 0.035 & 0.634 & 0.383 & 0.630 & 0.515 & 0.574 & 0.282 \\ \hline
UL & - & 0.000 & 0.004 & 3.381 & 0.990 & 0.524 & 0.257 & 0.560 & 0.498 & 0.325 & 0.258 \\ \hline
\multirow{2}{*}{TA} & 0.05 & 0.117 & 0.305 &  24.089 & 0.174 & 0.613 & 0.365 & 0.680 & 0.521 & 0.575 & 0.279 \\
 & 0.10 & 0.035 & 0.017 & 35.556 & 0.515 &  0.560 & 0.291 & 0.560 & 0.514 & 0.535 & 0.264 \\
\hline
\multirow{4}{*}{DP} & 0.0 & 0.000 & 0.005 & 45562.607 & 0.000 & 0.525 & 0.249 & 0.546 & 0.492 & 0.571 & 0.254 \\
 & 0.2 & 0.001 & 0.082 & 308.882 & 0.000 & 0.601 & 0.315 & 0.539 & 0.518 & 0.571 & 0.261 \\
 & 0.4 & 0.016 & 0.224 & 181.704 & 0.000 & 0.605 & 0.320 & 0.523 & 0.521 & 0.571 & 0.266 \\
 & 0.6 & 0.090 & 0.522 & 76.428 & 0.002 & 0.611 & 0.345 & 0.546 & 0.516 & 0.571 & 0.277 \\ \hline
\multirow{2}{*}{CD} & 0.50 & 0.017 & 0.172 & 158.187 & 0.042 & 0.592 & 0.319 & 0.630 & 0.504 & 0.562 & 0.273 \\
 & 0.25 & 0.089 & 0.333 & 52.202 & 0.056 & 0.611 & 0.346 & 0.644 & 0.516 & 0.576 & 0.278 \\ \hline \hline

\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}XXX \\ (Ours)\end{tabular}}
& 3.0 & 0.111 &  0.674 & 32.584 &  0.010 & 0.628 &          0.377 &  0.620 &       0.519 &   0.575 &      0.283 \\
& 10.0 & 0.019 &  0.450 & 65.591 &  0.005 & 0.626 &          0.373 &  0.620 &       0.520 &   0.575 &      0.282 \\
& 30.0 & 0.013 &  0.437 & 64.594 &  0.005 & 0.626 &          0.367 &  0.620 &       0.519 &   0.575 &      0.283 \\ \hline
\end{tabular}
\caption{\textbf{The performance of baseline methods and our methods on NLU benchmarks and open-ended generation metrics.} The coefficient are defined in Section \ref{baselines}. The coefficient for TA is the subtraction coefficient $\beta$. The coefficient for CD is the contrastive coefficient $\alpha$. The coefficient for DP is the DP coefficient $\lambda$. And, the coefficient for XXX is the penalty strength $\gamma$. The experimental setup can be found in Section \ref{hyperparam_selection}. We note that sometimes a method (e.g., UL) has low MAUVE but also low perplexity. That is because it also has high repetition which leads the generated text to be more expected and thus lower perplexity as observed in \cite{}.}
\end{table*}
\label{NLU}
